A Comprehensive Survey of Small Language Models in the Era of Large Language Models: Techniques, Enhancements, Applications, Collaboration with LLMs, and Trustworthiness

Large language models (LLMs) have demonstrated emergent abilities in text generation, question answering, and reasoning, facilitating various tasks and domains. Despite their proficiency in various tasks, LLMs like PaLM 540B and Llama-3.1 405B face limitations due to large parameter sizes and computational demands, often requiring cloud API use which raises privacy concerns, limits real-time applications on edge devices, and increases fine-tuning costs. Additionally, LLMs often underperform in specialized domains such as healthcare and law due to insufficient domain-specific knowledge, necessitating specialized models. Therefore, Small Language Models (SLMs) are increasingly favored for their low inference latency, cost-effectiveness, efficient development, and easy customization and adaptability. These models are particularly well-suited for resource-limited environments and domain knowledge acquisition, addressing LLMs' challenges and proving ideal for applications that require localized data handling for privacy, minimal inference latency for efficiency, and domain knowledge acquisition through lightweight fine-tuning. The rising demand for SLMs has spurred extensive research and development. However, a comprehensive survey investigating issues related to the definition, acquisition, application, enhancement, and reliability of SLM remains lacking, prompting us to conduct a detailed survey on these topics. The definition of SLMs varies widely, thus to standardize, we propose defining SLMs by their capability to perform specialized tasks and suitability for resource-constrained settings, setting boundaries based on the minimal size for emergent abilities and the maximum size sustainable under resource constraints. For other aspects, we provide a taxonomy of relevant models/methods and develop general frameworks for each category to enhance and utilize SLMs effectively.

==> sections/2.existing_slm.tex <==

\section{Review of Existing Small Language Models}
% \subsection{Early Pre-trained Models}


% \subsection{Evolved SLMs from Large Language Models}


==> sections/model/model_cards.tex <==

%%%StableLM 2 1.6B~\cite{bellagente2024stable,StableLM-3B-4E1T}, 2024.2, 2024.10
Stable LM 2 1.6B~\cite{bellagente2024stable}, a 1.6 billion parameter decoder-only model, is pre-trained on 2 trillion tokens from multilingual and code datasets. StableLM-3B-4E1T~\cite{StableLM-3B-4E1T}, a 3 billion parameter model, utilizes 1 trillion tokens from English and code datasets. Both models incorporate data from diverse sources such as Falcon RefinedWeb extract~\cite{penedo2023refinedweb}, RedPajama-Data~\cite{together2023redpajama}, The Pile (excluding Books3)~\cite{gao2020pile}, StarCoder~\cite{listarcoder}, and CulturaX's OSCAR corpora~\cite{nguyen2024culturax}. They are designed for foundational use and fine-tuning for specific applications.
Stable LM 2 is evaluated for zero-shot and few-shot capabilities across benchmarks, significantly outperforming other base models and surpassing Microsoft’s Phi-1.5 while trailing the larger Phi-2.0 in few-shot accuracy, as detailed in Table \ref{tab:results_mmlu_stablelm}. It also excels in English and machine-translated LAMBADA evaluations and performs competitively against Google’s Gemma 2B. In the MT-Bench, Stable LM 2 shows robust conversational skills, outdoing models like Phi-2, Gemma 2B, and TinyLLaMA 1.1B, despite its smaller size compared to the Mistral 7B Instruct v0.2, as shown in Table \ref{tab:results_mtbench_stablelm}.

\begin{table}[h]
\centering
\caption{Comparison of Open LLM leaderboard evals. \dag\ denotes aligned models. Note that in this table, we marked the Phi series of models \cite{26} as aligned. While we acknowledge that they may have only been pre-trained, by the nature of the training data used, and the self-disclaimed intended use for QA and chat formats, we believe this to be a fair statement~\cite{bellagente2024stable}.}
\label{tab:results_mmlu_stablelm}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Size} & \textbf{Avg} & \textbf{ARC} & \textbf{HS} & \textbf{MMLU} & \textbf{TQA} & \textbf{Wino} & \textbf{GSM} \\ \hline
phi-2\dag & 2.8B & 61.3 & 61.1 & 75.1 & 58.1 & 44.5 & 74.4 & 54.8 \\ \hline
stablelm-2-zephyr-1\_6b\dag & 1.6B & 49.7 & 43.3 & 69.3 & 41.8 & 45.6 & 63.6 & 34.8 \\ \hline
phi-1\_5\dag & 1.5B & 47.7 & 42.9 & 69.1 & 43.9 & 40.9 & 72.2 & 12.4 \\ \hline
stablelm-3b-4e1t & 2.7B & 46.6 & 46.6 & 75.9 & 45.2 & 37.2 & 71.2 & 3.3 \\ \hline
Qwen-1.5-1.8B & 1.8B & 46.6 & 37.9 & 61.4 & 46.7 & 39.4 & 60.3 & 33.6 \\ \hline
gemma-2b & 2.5B & 45.5 & 42.5 & 71.7 & 30.4 & 66.8 & 74.1 & 17.4 \\ \hline
stablelm-2-1\_6b & 1.6B & 45.3 & 43.3 & 70.5 & 38.9 & 36.8 & 64.6 & 17.4 \\ \hline
gemma-2b-it\dag & 2.5B & 42.7 & 43.9 & 62.7 & 37.6 & 45.8 & 60.9 & 5.5 \\ \hline
open\_llama\_3b & 3B & 40.3 & 39.9 & 71.6 & 27.1 & 34.8 & 67.0 & 0.9 \\ \hline
falcon-rw-1b & 1.3B & 37.1 & 35.1 & 63.6 & 25.3 & 35.9 & 62.0 & 0.5 \\ \hline
TinyLlama-1.1B & 1.1B & 36.4 & 33.9 & 60.3 & 26.0 & 37.3 & 59.5 & 1.4 \\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{MT-Bench results~\cite{bellagente2024stable}}
\label{tab:results_mtbench_stablelm}
\begin{tabular}{|l|c|c|}
\hline
\textbf{Model} & \textbf{Size} & \textbf{MT-Bench} \\ \hline
Mistral-7B-Instruct-v0.2 & 7B & 7.61 \\ \hline
Llama2-Chat & 70B & 6.86 \\ \hline
stablelm-zephyr-3b & 3B & 6.64 \\ \hline
MPT-30B-Chat & 30B & 6.39 \\ \hline
stablelm-zephyr-1.6b & 1.6B & 5.42 \\ \hline
Qwen-1.5-1.8B-Chat & 1.8B & 5.29 \\ \hline
gemma-2b-it & 2.5B & 5.19 \\ \hline
Falcon-40B-Instruct & 40B & 5.17 \\ \hline
dolphin-2.6-phi-2 & 2.7B & 4.93 \\ \hline
phi-2 & 2.7B & 4.29 \\ \hline
TinyLlama-1.1B-Chat-v1.0 & 1.1B & 3.46 \\ \hline
\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Pic/model/downloads_stablelm_last_month.pdf}
    \caption{StableLM-2 Downloads in the Last Month Across Various Model Sizes.}
    \label{fig:downloads-stablelm}
\end{figure}

% downloads amount of stablelm-2:
% 1.6B 18.6k
% 3B 52.7k
% 12B 3.41k

%%%


%%% Galactica-1.3B https://huggingface.co/facebook/galactica-1.3b, 2022.11, mini (125M), base (1.3B), standard (6.7B), large (30B), huge (120B)
The GALACTICA~\cite{taylor2022galactica}, developed by Meta AI's Papers with Code team, are trained on a 106 billion token scientific corpus to perform a variety of scientific tasks such as citation prediction, scientific QA, mathematical reasoning, summarization, document generation, molecular property prediction, and entity extraction. These models range from 125M to 120B parameters and are intended for researchers focusing on applying language models to the scientific domain. The training data encompasses open-access scientific papers, textbooks, websites, encyclopedias, and other knowledge-based resources.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Pic/model/downloads_galactica_last_month.pdf}
    \caption{Galactica Downloads in the Last Month Across Various Model Sizes.}
    \label{fig:downloads}
\end{figure}

Figure \ref{fig:downloads} displays the number of downloads last month for different Galactica model sizes. Notably, the 1.3B model is the most downloaded, indicating a higher popularity for models with sub-billion parameters among the public.
%%%


%%%% Gemma, learn from https://developers.googleblog.com/zh-hans/gemma-explained-new-in-gemma-2/
Gemma~\cite{team2024gemma, team2024gemma2, team2024codegemma} is a series of open-weight LLMs ranging from 2B to 27B versions. Gemma 1 features 2B and 7B models, while Gemma 2 extends to 2B, 9B, and 27B. CodeGemma, optimized for coding tasks, is fine-tuned on over 500 billion code-related tokens and includes a text interpolation feature. RecurrentGemma, in 2B and 9B versions, combines gated linear recurrences with local sliding window attention for enhanced processing of long contexts. Notably, the 2B Gemma 2 model excels in conversational AI and outperforms GPT-3.5 models in chatbot performance. 

%%%%


%%%% BLOOM, learn from https://developer.volcengine.com/articles/7387286618556039218, ALiBi \cite{press2022train}, Embedding LayerNorm \cite{dettmers2022gpt3}
BLOOM~\cite{le2023bloom,muennighoff2023crosslingual}, developed by BigScience, is trained on a ROOTS~\cite{laurenccon2022bigscience} corpus of 46 natural and 13 programming languages. Following pre-training, the models undergo large-scale multi-task instruction tuning to enhance zero-shot generalization, resulting in BLOOMZ. Available model sizes range from 560M to 176B.
%%%%



% General
% LLaMa, LLaMa 2, LLaMa 3, Falcon \cite{almazrouei2023falcon}, MPT-7B \cite{mosaicml2023introducing}， RPJ-INCITE \cite{together2023redpajama}， Orca 2 \cite{mitra2023orca}等模型都提供了7B或者相当的LM版本。

%%%% Phi Family
\textbf{Phi Family} Phi-1~\cite{gunasekar2023textbooksneed}, a Transformer with 1.3 billion parameters, specializes in basic Python coding. It trains on Python code from The Stack v1.2\footnote{https://huggingface.co/datasets/bigcode/the-stack}, StackOverflow Q\&A content\footnote{https://archive.org/download/stackexchange}, competition entries from code\_contests\footnote{https://github.com/deepmind/code\_contests}, and synthetic materials generated by gpt-3.5-turbo-0301. Although smaller than many modern LLMs, Phi-1 achieves over 50\% accuracy on the HumanEval Python coding benchmark.
Phi-1.5~\cite{li2023textbooksneediiphi15}, a Transformer with 1.3 billion parameters, uses the same training data as Phi-1, enhanced with additional NLP synthetic texts. It approaches state-of-the-art performance in benchmarks on common sense, language understanding, and logical reasoning among models with fewer than 10 billion parameters. Phi-1.5 can write poems, draft emails, create stories, summarize texts, write Python code (such as downloading a Hugging Face transformer model), etc.
Phi-2~\cite{javaheripi2023phi}, a Transformer with 2.7 billion parameters, builds on the data sources of Phi-1.5, adding NLP synthetic texts and curated websites for safety and educational value. It nearly reaches state-of-the-art performance in benchmarks for common sense, language understanding, and logical reasoning among models with fewer than 13 billion parameters.
The Phi-3 series~\cite{abdin2024phi} includes various models like phi-3-mini (3.8 billion parameters), phi-3-small (7 billion), and phi-3-medium (14 billion), trained on a scaled-up dataset of filtered web and synthetic data, with enhancements for safety and chat formats. The phi-3.5 series introduces multilingual, multimodal, and long-context capabilities. Phi-3.5-MoE, a 16 x 3.8B mixture of expert models with 6.6 billion active parameters, outperforms comparable open-source models in language, math, and coding tasks. Phi-3.5-Vision (4.2 billion), based on phi-3.5-mini, excels in reasoning across various image and text combinations.
% phi-3 downloads
% 3.8B 1.65M+242k
% 7B 24.1k+20k
% 14B 30.2k+44.9k

% 另一个版本的介绍
The development of the Phi-series models \cite{li2023textbooksneediiphi15, javaheripi2023phi, abdin2024phi, Trufinescu2024} marks a major milestone for SLMs, demonstrating strong performance relative to both similarly sized models and larger ones, 
especially in question-answering (QA) tasks suited for edge devices. This strong performance is attributed to the emphasis on high-quality training data, particularly "textbook-quality" material. The training data includes synthetic datasets designed to teach common sense and general knowledge across various domains, such as science and daily activities. Additionally, the corpus is enhanced with carefully filtered web data based on its educational value, creating a rich and effective training environment.
Notably, Phi-2 (2.7B parameters) \cite{javaheripi2023phi}, Phi-3-mini (3.8B parameters) \cite{abdin2024phi}, and Phi-3.5-mini (3.8B parameters) \cite{Trufinescu2024} have excelled on several open-domain reasoning benchmarks.
Phi-2 achieved comparable performance (59.2\%) on the BBH benchmark \cite{suzgun2022challenging}, closely matching larger models like Llama-2 70B (66.5\%) \cite{touvron2023llama2} and Mistral (57.2\%) \cite{jiang2023mistral}.
On the PIQA dataset \cite{bisk2020piqa}, Phi-2 (68.8\%) outperformed models with more parameters, such as Llama-2 7B (62.2\%) and Mistral (66.4\%), excelling in commonsense reasoning. 
Phi-3-mini also performed well on the BoolQ benchmark \cite{clark2019boolq}, achieving a score of 77.1\%, comparable to GPT-3.5 Turbo (79.1\%) and Mistral-8x7B (76.6\%). 
Despite having roughly half the parameters, Phi-3.5-mini surpassed models like Mistral-7B-Instruct in six out of nine QA benchmarks (ARC-Challenge \cite{clark2018think}, PIQA \cite{mihaylov2018can}, WinoGrande \cite {sakaguchi2021winogrande}, SIQA \cite{bauer2021identifyalignintegratematching}, BooIQ \cite{clark2019boolq}, GPQA \cite{rein2023gpqagraduatelevelgoogleproofqa}, HellasSwag \cite{zellers2019hellaswag}, OpenBookQA \cite{mihaylov2018can}, TruthfulQA \cite{lin2022truthfulqa}) and outperformed Llama 3.1-8B in five out of nine \cite{Trufinescu2024}. 

%%%%


The \textbf{Llama 3} \cite{dubey2024llama} and \textbf{Llama 3.2} \footnote{https://ai.meta.com/blog/llama-3-2-connect-2024-vision-edge-mobile-devices/} series introduce powerful, customizable models optimized for multilingual tasks, reasoning, coding, and tool usage. The flagship Llama 3 \cite{dubey2024llama} model, with 405B parameters and a 128K context window, performs on par with leading models like GPT-4 across various benchmarks. Llama 3.2 adds smaller, lightweight models (1B and 3B parameters) and vision models (11B and 90B parameters) that are specifically optimized for edge and mobile deployment. These models excel in tasks like summarization, instruction following, and tool calling, while being efficient enough to run on devices like Qualcomm and MediaTek hardware. Key techniques like structured pruning and knowledge distillation were applied to the smaller 1B and 3B models, reducing their size while retaining strong performance by transferring knowledge from larger Llama 3.1 models (8B and 70B). As a result, Llama 3.2 models outperform competitors like Gemma 2 \cite{team2024gemma2} and Phi 3.5-mini in tasks such as rewriting and instruction following, making them ideal for on-device AI applications that prioritize privacy and efficiency.

\textbf{Gemma} \cite{team2024gemma} and \textbf{Gemma 2}\cite{team2024gemma2}: The Gemma family of lightweight, open models, based on Google's Gemini research, includes two primary sizes: 2B and 7B parameters. These models are optimized for a range of deployment environments, with the 2B model suited for CPU and on-device tasks and the 7B model designed for GPU and TPU. Both models demonstrate strong performance across various text-based tasks and safety benchmarks, outperforming similar-sized models in many cases. Built on a Transformer architecture, Gemma employs Multi-Query Attention (for the 2B model) and full multi-head attention (for the 7B model), as well as Rotary Positional Embeddings (RoPE) and GeGLU activations. Gemma 2 expands this series with models ranging from 2B to 27B parameters, incorporating knowledge distillation to enhance performance even further. The 9B and 27B models employ deeper architectures and grouped-query attention (GQA), showing competitive performance with models twice their size. Across a wide range of benchmarks, including reasoning, mathematics, and coding, Gemma models excel while maintaining a focus on safety and responsible deployment.

\textbf{Mistral 7B} \footnote{https://mistral.ai/news/announcing-mistral-7b/} is a highly advanced 7.3 billion parameter language model that excels in performance despite its compact size. Using innovative techniques like Grouped-query attention (GQA) and Sliding Window Attention (SWA), it efficiently handles long sequences while reducing computational costs. Mistral 7B surpasses Llama 2 13B on all major benchmarks and rivals Llama 34B, particularly in reasoning, comprehension, and code-related tasks. It achieves near-parity with CodeLlama 7B on code performance while excelling in English tasks. The model's architecture integrates improvements such as FlashAttention and optimizations via xFormers, providing a 2x speed boost for sequences up to 16k tokens with a sliding window of 4k. This mechanism also allows it to manage memory more effectively, saving cache space during inference without sacrificing quality. Additionally, Mistral 7B is easily fine-tuned for various applications, including chat. The fine-tuned "Mistral 7B Instruct" model outperforms all other 7B models and rivals 13B chat models in tasks like MT-Bench. Available under the Apache 2.0 license, Mistral 7B can be deployed across various platforms, including cloud services and HuggingFace, making it accessible for diverse applications. With its ability to perform on par with models three times its size, Mistral 7B offers significant memory savings and faster inference, positioning it as one of the most efficient and powerful models at its scale.


\textbf{OpenELM} \cite{mehta2024openelm} is an efficient language model family based on a transformer architecture that uses a novel layer-wise scaling strategy for more effective parameter allocation across layers. This scaling method optimizes the transformer layers by progressively increasing the dimensions of attention heads and feed-forward modules from the input layers to the output layers. The result is a performance improvement of 2.36\% compared to OLMo, with OpenELM using only half the pre-training tokens, making it highly efficient in resource use. OpenELM is pre-trained on public datasets such as RefinedWeb, RedPajama, and PILE, totaling 1.8 trillion tokens. It employs pre-normalization with RMSNorm and rotary positional embeddings for encoding positional information, and it uses grouped-query attention (GQA) instead of traditional multi-head attention. This model is made fully open, providing pre-trained checkpoints, training logs, pre-training configurations, and inference code. This transparency enables reproducibility and further research in large language model (LLM) development. OpenELM models can be trained and fine-tuned using a comprehensive open framework released alongside the models. The largest OpenELM model, consisting of 1.1 billion parameters, demonstrates enhanced accuracy and efficiency in performance evaluations, competing effectively with other LLMs.

%%% Qwen: Alibaba. Qwen 1. https://huggingface.co/alibaba/Qwen-1, 2023.12. Alibaba. Qwen 1.5. https://huggingface.co/alibaba/Qwen-1.5, 2024.04. Alibaba. Qwen 2. https://huggingface.co/alibaba/Qwen-2, 2024.06.  Alibaba. Qwen 2.5. https://qwenlm.github.io/blog/qwen2.5/, 2024.10.
% Qwen~\cite{bai2023qwen}, 2023.9
Qwen-1~\cite{bai2023qwen} is the [1.8B, 7B, 14B, 72B]-parameter version of the large language model series, Qwen (abbr. Tongyi Qianwen), proposed by Aibaba Cloud. Qwen-1.8B is a Transformer-based large language model, which is pretrained on a large volume of data, including web texts, books, codes, etc. Additionally, based on the pretrained Qwen-1.8B, we release Qwen-1.8B-Chat, a large-model-based AI assistant, which is trained with alignment techniques. 
Qwen1.5 is the beta version of Qwen2, a transformer-based decoder-only language model pretrained on a large amount of data. In comparison with the previous released Qwen, the improvements include:
8 model sizes, including 0.5B, 1.8B, 4B, 7B, 14B, 32B and 72B dense models, and an MoE model of 14B with 2.7B activated;
Significant performance improvement in Chat models;
Multilingual support of both base and chat models;
Stable support of 32K context length for models of all sizes
\textbf{Qwen2} \cite{yang2024qwen2} is a powerful family of large language models and multimodal models, including dense models and Mixture-of-Experts (MoE) models. The Qwen2 series features models ranging from 0.5 billion to 72 billion parameters, significantly outperforming many previous open-weight models in tasks such as language understanding, generation, multilingual proficiency, coding, and mathematical reasoning. Pretrained and instruction-tuned models of 5 sizes, including Qwen2-0.5B, Qwen2-1.5B, Qwen2-7B, Qwen2-57B-A14B, and Qwen2-72B;
Having been trained on data in 27 additional languages besides English and Chinese;
State-of-the-art performance in a large number of benchmark evaluations;
Significantly improved performance in coding and mathematics;
Extended context length supports up to 128K tokens with Qwen2-7B-Instruct and Qwen2-72B-Instruct.
In terms of Qwen2.5 (Qwen2.5: 0.5B, 1.5B, 3B, 7B, 14B, 32B, and 72B), the language models, all models are pre-trained on our latest large-scale dataset, encompassing up to 18 trillion tokens. Compared to Qwen2, Qwen2.5 has acquired significantly more knowledge (MMLU: 85+) and has greatly improved capabilities in coding (HumanEval 85+) and mathematics (MATH 80+). Additionally, the new models achieve significant improvements in instruction following, generating long texts (over 8K tokens), understanding structured data (e.g., tables), and generating structured outputs, especially JSON. Qwen2.5 models are generally more resilient to the diversity of system prompts, enhancing role-play implementation and condition-setting for chatbots. Like Qwen2, the Qwen2.5 language models support up to 128K tokens and can generate up to 8K tokens. They also maintain multilingual support for over 29 languages, including Chinese, English, French, Spanish, Portuguese, German, Italian, Russian, Japanese, Korean, Vietnamese, Thai, Arabic, and more. Below, we provide basic information about the models and details of the supported languages.
% 0.5B 74.8k+75k+3.26k+4.14k
% 1.5B 16.3k+32M
% 3B 11.8k+79.2k+5.62k+1.39k
% 7B 14.8k+80.7k+9.89k+3.55k+4.92k+1.76k
% 14B 10.4k+42.1k+4.31k+2.77k+1.47k
% 32B 8.18k+42.5k+4.86k+7.71k+2.53k+2.03k
% 72B 5.43k+106k+7.48k+7.49k+4.68k+3.25K
% 
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.5\linewidth]{Pic/model/downloads_qwen2.5_last_month.pdf}
    \caption{Qwen2.5 Downloads in the Last Month Across Various Model Sizes.}
    \label{fig:downloads_qwen}
\end{figure}
%%%

\textbf{Mamba} \cite{gu2023mamba} and \textbf{Mamba-2} \cite{dao2024transformers} are state-of-the-art Linear-Time Sequence Models designed for efficient sequence processing and superior performance across tasks such as language, audio, and genomics. These models leverage Selective State Space Models (SSMs) to replace traditional attention and MLP blocks, resulting in faster inference (up to 5× faster than Transformers) and efficient handling of long sequences up to 1M tokens. The models, including Mamba-130M, Mamba-2.8B, and Mamba2-2.7B, were trained on large datasets such as the Pile (300B tokens) and SlimPajama (600B tokens). Mamba-2 introduces the "Structured State Space Duality" (SSD), providing a 2-8× speedup over traditional architectures. With a throughput 5× higher than similarly-sized Transformers, models like Mamba-3B and Mamba2-2.7B achieve state-of-the-art performance on language modeling and reasoning tasks, outperforming models like Pythia-2.8B and even Pythia-6.9B. These models are highly efficient for real-world applications that require long-context reasoning and provide a competitive alternative to traditional Transformer-based architectures.

\textbf{SAMBA} \cite{ren2024samba} is a hybrid neural architecture designed to efficiently handle language modeling tasks with unlimited context length. It combines selective State Space Models (SSMs), Mamba layers, and Sliding Window Attention (SWA) to capture time-dependent semantics and efficiently process long-term context. SAMBA scales up to 3.8B parameters, pre-trained on 3.2T tokens, achieving superior performance on tasks such as MMLU, HumanEval, and GSM8K compared to models with up to 8B parameters. Notably, SAMBA maintains linear decoding time complexity and can extrapolate up to 1M context lengths while retaining memory recall. The 3.8B model achieves substantial improvements in prompt processing and decoding throughput, especially in long-context summarization tasks. Structured pruning and fine-tuning techniques allow SAMBA to efficiently recall memory over extended sequences, demonstrating its effectiveness across various benchmarks. By balancing Mamba's strengths in recurrent structure capturing with the precision of attention mechanisms, SAMBA is positioned as a robust architecture for tasks requiring extensive context understanding and memory retention.

\textbf{Zamba} \cite{glorioso2024zamba} is a 7B SSM-Transformer hybrid that uses a Mamba backbone with a global shared attention module to enhance memory recall and efficiency in handling long sequences. Trained on 1T tokens from open web datasets, Zamba demonstrates competitive performance relative to models of similar scale, such as LLaMA2, outperforming many models on tasks involving common-sense reasoning, language understanding, and in-context learning. Zamba’s architecture minimizes the parameter cost while retaining the ability to efficiently process long-context sequences, making it faster and more memory-efficient during inference compared to Transformer models. Zamba was pretrained in two phases: the first on standard web datasets, and the second involving an annealing phase using high-quality instructional datasets. Performance benchmarks show Zamba excels in memory-intensive tasks, with performance comparable to Transformer-based models while requiring less computational resources. Additionally, Zamba is particularly efficient in in-context learning due to its shared global attention mechanism. \textbf{Zamba2-2.7B} \footnote{https://huggingface.co/Zyphra/Zamba2-2.7B} further extends this architecture, incorporating improvements such as Mamba2 blocks, two interleaved shared attention blocks, and the use of LoRA projectors to enable specialized depth for the MLP layers. It was pre-trained on 3T tokens and annealed with an additional 100B high-quality tokens, achieving state-of-the-art performance for models under 3B parameters. Its low memory footprint and high inference speed make Zamba2-2.7B suitable for on-device applications. However, it has not been fine-tuned for instruction-following tasks and should be approached with caution regarding potential harmful outputs due to its lack of moderation.

\textbf{Liquid Foundation Models (LFMs)}\footnote{https://www.liquid.ai/liquid-foundation-models} are a new series of general-purpose AI models designed from first principles, focusing on state-of-the-art performance across multiple scales while maintaining memory efficiency. The initial release includes three models: a 1.3B dense model for resource-constrained environments, a 3.1B dense model optimized for edge deployment, and a 40.3B Mixture of Experts (MoE) model designed for more complex tasks. These models are built on a foundation of dynamic learning systems, combining advances from dynamical systems, signal processing, and numerical linear algebra to efficiently handle sequential data. The LFM-1.3B model achieves leading scores across various benchmarks in the 1B parameter category, surpassing traditional GPT-based architectures. The LFM-3.1B model outperforms many models in the 3B-parameter range, including transformers, hybrids, and RNNs, and performs on par with Phi-3.5-mini while being 18.4\% smaller. Notably, LFMs are optimized for long-context tasks, offering a 32k token context length, which enhances performance for document summarization, context-aware chatbots, and retrieval-augmented generation (RAG). LFMs are designed for efficient inference on a variety of hardware platforms, including NVIDIA, AMD, Qualcomm, Cerebras, and Apple, and are suitable for applications in industries such as finance, biotechnology, and consumer electronics.

\textbf{MiniCPM} \cite{hu2024minicpm} is a series of Small Language Models (SLMs) designed to balance scalability and efficiency with high performance. The models come in two main configurations: a 2.4B and a 1.2B non-embedding parameter version. These models are developed to rival larger LLMs, achieving performance comparable to models in the 7B-13B parameter range, such as Llama2-7B and Mistral-7B, despite their smaller size. Key innovations in MiniCPM include the Warmup-Stable-Decay (WSD) learning rate scheduler, which optimizes training dynamics and enhances efficient scaling in both model size and data. This allows MiniCPM to efficiently pre-train with minimal data size requirements. The introduction of intermediate checkpoints also enables continuous training without retraining the entire model. The MiniCPM family consists of variants such as MiniCPM-DPO, MiniCPM-MoE, and MiniCPM-128K. Among them, the 2.4B MiniCPM-128K shows competitive or superior performance to other models, surpassing Mistral-7B and Llama-13B in multiple benchmarks, including MTBench. MiniCPM-MoE, with 4B activated parameters, achieves results on par with Llama2-34B, demonstrating its robustness in various tasks. Overall, MiniCPM’s efficient design, scalability, and impressive results in both 2B and 1B scale categories make it a powerful, resource-efficient alternative in the SLM landscape.

\textbf{Rene} \footnote{https://cartesia.ai/blog/on-device} is a highly efficient 1.3B parameter Small Language Model (SLM) designed for on-device use. It utilizes a hybrid architecture with alternating Mamba-2 and MLP layers, complemented by sliding-window attention (SWA) layers. Trained on 1.5 trillion tokens from the Dolma-1.7 dataset, Rene's architecture is tailored for resource-constrained environments, ensuring a fixed memory footprint and faster prefill times at inference. Rene demonstrates strong performance on several standard benchmarks, including common-sense reasoning tasks (COPA, WinoGrande, ARC-Easy, ARC-Challenge) and language understanding benchmarks (PIQA, HellaSwag, OpenBookQA, MMLU). It outperforms other SLMs like Apple's OpenELM (1.1B) and Google's recurrent Gemma (2B), marking a significant achievement for a recurrent architecture-based SLM in this parameter range. Rene supports native on-device usage through the Edge platform, which enables 8-bit and 4-bit quantization for faster inference with no quality loss. This model is part of Cartesia’s broader vision to build real-time multimodal intelligence optimized for every device, paving the way for next-generation hardware-optimized models.

\textbf{MINITRON} \cite{muralidharan2024compact} is a family of compressed language models derived from the Nemotron-4 15B LLM, using structured pruning and knowledge distillation. This approach allows for a compression factor of 2-4×, significantly reducing the model size and training costs. MINITRON models are available in 4B, 8B, and 15B parameter variants, and can be trained with up to 40× fewer tokens compared to full training from scratch, while maintaining performance on par with similarly-sized models. The model utilizes a combination of width, attention head, and MLP pruning, with the use of the Warmup-Stable-Decay (WSD) learning rate scheduler for efficient retraining. The pruning method allows MINITRON to achieve comparable or better performance than other community models, such as Mistral-7B, Gemma-7B, and LLaMA-2 7B/8B, while using significantly less training data. MINITRON-8B outperforms Nemotron-3 8B and is competitive with Mistral-7B, while MINITRON-4B compares favorably with models like Phi-2. These models provide a cost-efficient alternative to training from scratch while delivering state-of-the-art performance across language modeling tasks.

\textbf{Phi-3}: \cite{abdin2024phi} The Phi-3 family introduces multiple language models designed for on-device deployment, with the flagship model being phi-3-mini, a 3.8 billion parameter model trained on 3.3 trillion tokens. Despite its compact size, phi-3-mini achieves impressive performance, rivaling models like Mistral 8x7B and GPT-3.5, with scores of 69\% on MMLU and 8.38 on MT-bench. The Phi-3 models use a transformer decoder architecture with a default context length of 4K. The model is built on a scalable architecture from the Phi-2 model but has been expanded for robustness, safety, and chat format. To further enhance the series, Phi-3 includes phi-3-small (7B parameters), phi-3-medium (14B parameters), and a series of models under the phi-3.5 label, which feature Mixture of Experts (MoE) architecture. The phi-3.5-MoE model, with 6.6 billion active parameters and 16 expert networks, specializes in reasoning, math, and code tasks. Additionally, the phi-3.5-Vision model includes 4.2 billion parameters and is adept at handling both text and image inputs, excelling in multimodal applications. Phi-3 models support long-context tasks and are built for robust performance across multilingual tasks. With their compact size, these models can be deployed directly on mobile devices like iPhones. In fact, phi-3-mini was quantized to 4-bit precision, allowing it to run on an iPhone 14 with only 1.8GB of memory, achieving more than 12 tokens per second, which is groundbreaking for local, on-device AI applications.


% 2024.2 1. MobiLlama是一个通用SLM，从头训练，提出parameter sharing scheme, 大小是0.5B，0.8B。公开代码在 \footnote{https://github.com/ mbzuai-oryx/MobiLlama}。预训练数据集是1.2T tokens from LLM360 Amber dataset \cite{liu2023llm360}, 包括了Arxiv，Book， C4, Refined-Web, StarCoder, Stackexchange, Wikipedia数据源. 0.5B结构是2048隐藏层，中间MLP size是5632， 32个attention heads across 22 hidden layers, vocab size is 32000，窗口大小是2048. our 0.8B design increases the hidden dimension size to 2532 and the intermediate size to 11,080 while the rest of the configuration is the same. 为了进一步提高训练效率，我们采用了 flash-attention 机制，并遵循 LLaMA \cite{touvron2023llama} 模型建立的预训练超参数。训练机器20 GPU nodes each equipped with 8 NVIDIA A100 GPUs with 80 GB memory。在9个benchmark （HellaSway，TruthfulQA， MMLU, ARC_Challenge, CrowsPairs, PIQA, Race, SIQA, Sinogrande）上评估SLM的事实理解能力，知识水平，复杂推理能力，bias，阅读理解能力，解决歧义能力 \footnote{https://huggingface.co/spaces/open-llm-leaderboard/open_llm_leaderboard}。对 Hellaswag、ARC_Challenge、Winogrande 和 MMLU 进行 10、25、5 和 5 个样本评估，而对其余基准测试进行零样本评估。(Table \ref{tab:model_comparisons}) MobiLlama 0.5B 模型实现了卓越的性能，平均得分为 46.0，在九个基准测试的平均性能方面比 pythia-410m 高出 2.4%。(Table \ref{tab:efficiency_comparison}) MobiLlama performs favorably in terms of efficiency across different hardware platforms.
\textbf{MobiLlama} \cite{thawakar2024mobillama} is a general-purpose SLM designed from scratch, available in 0.5B and 0.8B configurations. Its source code is openly shared \footnote{https://github.com/mbzuai-oryx/MobiLlama}. Pre-trained on the 1.2T token LLM360 Amber dataset \cite{liu2023llm360}, it incorporates data from diverse sources including Arxiv, Book, C4, Refined-Web, StarCoder, StackExchange, and Wikipedia. The 0.5B model features 2048 hidden dimensions, 5632 MLP size, 32 attention heads, 32000 vocabulary size, and a 2048 sequence window. The 0.8B version increases hidden dimensions to 2532 and MLP size to 11,080, maintaining other configurations. Enhanced with flash-attention and trained on 20 GPU nodes each equipped with 8 NVIDIA A100 GPUs, MobiLlama has been benchmarked on nine platforms including HellaSwag \cite{zellers2019hellaswag}, TruthfulQA \cite{lin2022truthfulqa}, MMLU \cite{hendrycksmeasuring}, ARC\_Challenge \cite{clark2018think}, CrowsPairs \cite{nangia2020crows}, PIQA \cite{bisk2020piqa}, Race \cite{lai2017race}, SIQA \cite{sap2019social}, and Winogrande \cite{sakaguchi2021winogrande}, focusing on factual understanding, knowledge level, complex reasoning, bias detection, and reading comprehension \footnote{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard}. It excelled in limited-sample evaluations on Hellaswag, ARC\_Challenge, Winogrande, and MMLU, and zero-shot assessments on other benchmarks (Table \ref{tab:model_comparisons} and \ref{tab:large_base_comparison}). The MobiLlama 0.5B model achieved an average score of 46.0, outperforming many in its category. Its efficiency across various hardware platforms is detailed in Table \ref{tab:efficiency_comparison}. 
\begin{table}[!h]
\centering
\small
\caption{State-of-the-art comparisons with existing \( < 1B \) parameters models on nine benchmarks. In case of around 0.5B model series, our MobiLlama achieves a substantial gain of 2.4\% in terms of average performance on nine benchmarks. Further, our MobiLlama 0.8B model achieves an average score of 46.67.}
\label{tab:model_comparisons}
\begin{tabular}{lcccccccccc}
\hline
\textbf{Model Name} & \textbf{\#Params} & \textbf{HellaSwag} & \textbf{Truthfulqa} & \textbf{MMLU} & \textbf{Arc\_C} & \textbf{CrowsPairs} & \textbf{piqa} & \textbf{race} & \textbf{siqa} & \textbf{winogrande} \\
\hline
gpt-neo-125m        & 0.15B & 30.26 & 45.58 & 25.97 & 22.95 & 61.55 & 62.46 & 27.56 & 40.33 & 51.78 \\
tiny-starcoder      & 0.17B & 28.17 & 47.68 & 26.79 & 20.99 & 49.68 & 52.55 & 25.45 & 38.28 & 51.22 \\
cerberas-gpt-256m   & 0.26B & 28.99 & 45.98 & 26.83 & 22.01 & 60.52 & 61.42 & 27.46 & 40.53 & 52.49 \\
opt-350m            & 0.35B & 36.73 & 40.83 & 26.02 & 23.55 & 64.12 & 64.74 & 29.85 & 41.55 & 52.64 \\
megatron-gpt2-345m  & 0.38B & 39.18 & 41.51 & 24.32 & 24.23 & 64.82 & 66.87 & 31.19 & 40.28 & 52.96 \\
LiteLlama           & 0.46B & 38.47 & 41.59 & 26.17 & 24.91 & 62.90 & 67.73 & 28.42 & 40.27 & 49.88 \\
gpt-sw3-356m        & 0.47B & 37.05 & 42.55 & 25.93 & 23.63 & 61.59 & 64.85 & 32.15 & 41.56 & 53.04 \\
pythia-410m         & 0.51B & 40.85 & 41.22 & 27.25 & 26.19 & 64.20 & 67.19 & 30.71 & 41.40 & 53.12 \\
xglm-564m           & 0.56B & 34.64 & 40.43 & 25.18 & 24.57 & 62.25 & 64.85 & 29.28 & 42.68 & 53.03 \\
Lamini-GPT-LM       & 0.59B & 31.55 & 40.72 & 25.53 & 24.23 & 63.09 & 63.87 & 29.95 & 40.78 & 47.75 \\
\textbf{MobiLlama (Ours)} & \textbf{0.5B}  & \textbf{52.52} & \textbf{38.05} & \textbf{26.45} & \textbf{29.52} & \textbf{64.03} & \textbf{72.03} & \textbf{33.68} & \textbf{40.22} & \textbf{57.53} \\
\textbf{MobiLlama (Ours)} & \textbf{0.8B}  & \textbf{54.09} & \textbf{38.48} & \textbf{26.92} & \textbf{30.20} & \textbf{64.82} & \textbf{73.17} & \textbf{33.37} & \textbf{41.60} & \textbf{57.45} \\
\hline
\end{tabular}
\end{table}

\begin{table}[!h]
\centering
\small
\caption{Comprehensive comparisons with existing $<2B$ params fully open-source LLM models on 9 benchmarks. Our 1.2B \textit{large-base} model pre-trained on 1.2T tokens achieves superior performance compared to the recent OLMo 1.17B and TinyLlama 1.1B models, which are pre-trained on substantially larger data of 3T tokens.}
\label{tab:large_base_comparison}
\begin{tabular}{lccccccccccc}
\hline
\textbf{Model Name} & \textbf{\#Params} & \textbf{HellaSwag} & \textbf{Truthfulqa} & \textbf{MMLU} & \textbf{Arc\_C} & \textbf{CrowsPairs} & \textbf{piqa} & \textbf{race} & \textbf{siqa} & \textbf{winogrande} & \textbf{Average} \\
\hline
Boomer & 1B & 31.62 & 39.42 & 25.42 & 22.26 & 61.55 & 57.99 & 28.99 & 40.32 & 50.98 & 39.80 \\
Pythia-Dedup & 1B & 49.63 & 38.92 & 24.29 & 29.09 & 67.11 & 70.23 & 32.44 & 42.63 & 53.98 & 45.36 \\
Falcon-RW & 1B & 63.12 & 35.96 & 25.36 & 35.06 & 69.04 & 74.10 & 36.07 & 40.23 & 61.88 & 48.98 \\
TinyLlama & 1.1B & 60.22 & 37.59 & 26.11 & 33.61 & 70.60 & 73.28 & 36.45 & 41.65 & 59.18 & 48.74 \\
OLMo & 1.2B & 62.50 & 32.94 & 25.86 & 34.45 & 69.59 & 73.70 & 36.74 & 41.14 & 58.90 & 48.42 \\
Cerebras-GPT & 1.3B & 38.51 & 42.70 & 26.66 & 26.10 & 63.67 & 66.75 & 30.33 & 42.42 & 53.59 & 43.41 \\
Lamini & 1.3B & 38.05 & 36.43 & 28.47 & 26.62 & 64.62 & 67.89 & 33.39 & 43.19 & 50.59 & 43.25 \\
OPT & 1.3B & 54.50 & 38.67 & 24.63 & 29.60 & 70.70 & 72.47 & 34.16 & 42.47 & 59.74 & 47.43 \\
GPT-NEO & 1.3B & 48.49 & 39.61 & 24.82 & 31.31 & 65.67 & 71.05 & 34.06 & 41.81 & 57.06 & 45.98 \\
Pythia-Deduped & 1.4B & 55.00 & 38.63 & 25.45 & 32.59 & 67.33 & 72.68 & 34.64 & 42.68 & 56.90 & 47.32 \\
\textbf{large-base} & 1.2B & \textbf{62.99} & \textbf{35.90} & \textbf{24.79} & \textbf{34.55} & \textbf{68.49} & \textbf{75.57} & \textbf{35.31} & \textbf{41.96} & \textbf{62.03} & \textbf{49.06} \\
\hline
\end{tabular}
\end{table}


\begin{table}[!h]
\centering
\small
\caption{Comparison of efficiency and resource consumption on low-end hardware devices.}
\label{tab:efficiency_comparison}
\begin{tabular}{lcccp{2cm}p{2cm}p{2cm}p{1.4cm}}
\hline
\textbf{Platform} & \textbf{Model} & \textbf{\#Params} & \textbf{Precision} & \textbf{Avg Tokens/Sec} & \textbf{Avg Memory Consumption} & \textbf{Avg Battery Consumption /1k Tokens} & \textbf{CPU Utilization} \\ \hline
\multirow{4}{*}{RTX2080Ti} 
&Llama2 & 7B & bf16 & 14.85 & 27793 MB & 135.51 mAH & 31.62\% \\
&Phi2 & 2.7B & bf16 & 32.19 & 12071 MB & 59.13 mAH & 24.73\% \\
&large-base & 1.2B & bf16 & 50.61 & 6254 MB & 18.91 mAH & 18.25\% \\
&MobiLlama & 0.5B & bf16 & 63.38 & 3046 MB & 8.19 mAH & 14.79\% \\
\multirow{4}{*}{CPU-i7} \\
&Llama2 & 7B & 4bit & 5.96 & 4188 MB & 73.5 mAH & 49.16\% \\
&Phi2 & 2.7B & 4bit & 22.14 & 1972 MB & 27.36 mAH & 34.92\% \\
&large-base & 1.2B & 4bit & 29.23 & 1163 MB & 10.81 mAH & 30.84\% \\
&MobiLlama & 0.5B & 4bit & 36.32 & 799 MB & 4.86 mAH & 24.64\% \\
\multirow{4}{*}{Snapdragon-685} \\
&Llama2 & 7B & 4bit & 1.193 & 4287 MB & 10.07 mAH & 77.41\% \\
&Phi2 & 2.7B & 4bit & 2.882 & 1893 MB & 14.61 mAH & 56.82\% \\
&large-base & 1.2B & 4bit & 6.687 & 780 MB & 6.00 mAH & 17.15\% \\
&MobiLlama & 0.5B & 4bit & 7.021 & 770 MB & 5.32 mAH & 13.02\% \\
\hline
\end{tabular}
\end{table}
% MobileLLM 认为移动设备上应该承担1B以下的模型。首先，移动应用程序不应超过 DRAM 的 10%，1B模型需要占用1GB with int8 占用内存8-12GB的手机的10%左右。通过使用低于 10 亿的模型，例如仅消耗 0.035 J/token 的 350M 8 位模型，iPhone （充满电的 iPhone，大约有 50kJ 能量）可以支持一整天的会话使用。鉴于这些考虑，动机是参数小于 10 亿的 LLM 的设计和实现。本文提出几个特定于1B模型从头训练的技术（SwiGLU FFN， deep and thin architectures, embedding sharing, and grouped query attention）在1T tokens语料上。在零样本常识推理任务上评估预训练模型，包括 ARC-easy、ARCchallenge \cite{clark2018think}、BoolQ \cite{clark2019boolq}、PIQA  \cite{bisk2020piqa}、 SIQA \cite{sap2019social}、HellaSwag  \cite{zellers2019hellaswag}、OpenBookQA \cite{mihaylov2018can}、WinoGrande  \cite{sakaguchi2021winogrande}，以及使用TQA \cite{joshi2017triviaqa}和 RACE 数据集\cite{lai2017race}。实验结果正面这几个技术的有效性。同时在下游任务API Call上微调测试微调在下游任务的有效性。为了使 LM 适应此任务，创建了一个包含 5000 个训练样本和 2500 个测试样本的合成数据集。表 \ref{tab:MobileLLM_api_calling_scores} 显示，MobileLLM-350M 表现出与 LLaMA-2-7B 相当的意图和结构精确匹配分数，其中高意图分数表明对用户打算调用的 API 的正确预测，而结构精确匹配分数反映了预测 API 函数内内容的熟练程度。
\textbf{MobileLLM} \cite{liu2024mobilellm} recommends deploying models with less than 1 billion parameters on mobile devices, targeting no more than 10\% of a device's DRAM—suitable for a 1B model requiring about 1GB on phones with 8-12GB memory. Employing models under 1 billion parameters, like a 350M model consuming only 0.035 J/token, allows an iPhone with around 50kJ energy to support all-day usage. Motivated by these factors, the paper advocates designing and implementing LLMs with less than 1 billion parameters, using techniques such as SwiGLU FFN, deep and thin architectures, embedding sharing, and grouped query attention trained on a 1 trillion token corpus. The models are evaluated on zero-shot commonsense reasoning tasks including ARC-Easy, ARC-Challenge, BoolQ, PIQA, SIQA, HellaSwag, OpenBookQA, WinoGrande, TQA, and RACE. Results validate the effectiveness of these techniques. Additionally, fine-tuning experiments on the downstream task of API Calls are conducted using a synthetic dataset with 5,000 training and 2,500 test samples, where MobileLLM-350M matches LLaMA-2-7B in intent and structural precision scores, indicating accurate predictions of intended API calls and proficiency in predicting API function contents.
\begin{table}[t]
\centering
\caption{API Calling Evaluation Score}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Model} & \textbf{EM\_intent} & \textbf{EM\_structure} & \textbf{R1} & \textbf{RL} \\ 
\hline
OPT-350M & 56.1 & 38.6 & 37.1 & 35.3 \\
Pythia-410M & 62.2 & 44.7 & 43.1 & 41.1 \\
BLOOM-560M & 64.7 & 37.9 & 36.9 & 34.6 \\
MobileLLM-350M & 65.3 & 48.8 & 46.8 & 44.6 \\
LLaMA-v2 7B & 62.8 & 50.9 & 56.5 & 54.3 \\
\hline
\end{tabular}
\label{tab:MobileLLM_api_calling_scores}
\end{table}
% 2024, TinyLLama \cite{zhang2024tinyllamaopensourcesmalllanguage}, code is here \footnote{https://github.com/jzhang38/TinyLlama}. 当使用更多数据进行训练时，较小的模型可以匹配甚至超越较大的模型。使用多达 3 万亿个令牌训练具有 1.1B 个参数的仅 Transformer 解码器模型（Vaswani 等人，2017）。这是第一次尝试使用如此大量的数据来训练具有 1B 参数的模型。预训练数据来源：SlimPajama \cite{cerebras2023slimpajama} 和 StarCoder \cite{listarcoder}的训练数据。遵循Llama 模型系列，模型基于仅解码器 Transformer，架构包括positional embedding, pre-norm and RMSNorm \cite{zhang2019root}, SwiGLU \cite{shazeer2020glu}, Grouped-query Attention \cite{ainslie2023gqa}, 优化技术包括Fully Sharded Data Parallel (FSDP), Flash Attention \cite{daoflashattention}, xFormers \cite{xFormers2022}。22层，5632维度，32000词表大小，窗口大小2048。基于lit-gpt\cite{litgpt-2023}构建框架。使用 16 个 A100-40G GPU 预训练 TinyLlama。为了了解 TinyLlama 的常识推理能力，考虑以下任务：Hellaswag \cite{zellers2019hellaswag}、OpenBookQA \cite{mihaylov2018can}、WinoGrande \cite{sakaguchi2021winogrande}、ARC-Easy 和 ARC -Challenge \cite{clark2018think}、BoolQ \cite{clark2019boolq}和 PIQA \cite{bisk2020piqa}。采用语言模型评估框架\cite{gao10256836framework}来评估模型。使用 InstructEval 基准(Massive Multitask Language Understanding (MMLU) \cite{hendrycksmeasuring}, BIG-Bench Hard (BBH) \cite{suzgun2022challenging}, Discrete Reasoning Over Paragraphs (DROP) \cite{dua2019drop}, HumanEval \cite{zheng2023codegeex})评估 TinyLlama 解决问题的能力。TinyLlama demonstrates better problem-solving skills compared to existing models (OPT-1.3B \cite{zhang2022opt}, Pythia-1.0B, and Pythia-1.4B \cite{pmlr-v202-biderman23a}).
\textbf{TinyLLama} \cite{zhang2024tinyllamaopensourcesmalllanguage}, accessible at \footnote{https://github.com/jzhang38/TinyLlama}, is a 1.1 billion-parameter model trained with up to 3 trillion tokens on a pure Transformer decoder \cite{vaswani2017attention}. It uses pre-training data from SlimPajama \cite{cerebras2023slimpajama} and StarCoder \cite{listarcoder}, incorporating architectural features like positional embeddings, RMSNorm \cite{zhang2019root}, SwiGLU \cite{shazeer2020glu}, and Grouped-query Attention \cite{ainslie2023gqa}. Optimization utilizes techniques such as FSDP, Flash Attention \cite{daoflashattention}, and xFormers \cite{xFormers2022}. Configurations include 22 layers, 5632 dimensions, a 32000 vocabulary size, and a 2048 sequence window. Built on the lit-gpt framework \cite{litgpt-2023} and pre-trained using 16 NVIDIA A100-40G GPUs. Assessed on tasks like Hellaswag \cite{zellers2019hellaswag}, OpenBookQA \cite{mihaylov2018can}, WinoGrande \cite{sakaguchi2021winogrande}, ARC-Easy and ARC-Challenge \cite{clark2018think}, BoolQ \cite{clark2019boolq}, and PIQA \cite{bisk2020piqa}, employing an evaluation framework \cite{gao10256836framework}. Additional evaluations used InstructEval (MMLU \cite{hendrycksmeasuring}, BIG-Bench Hard (BBH) \cite{suzgun2022challenging}, DROP \cite{dua2019drop}, HumanEval \cite{zheng2023codegeex}), where TinyLlama excelled over models like OPT-1.3B \cite{zhang2022opt}, Pythia-1.0B, and Pythia-1.4B \cite{pmlr-v202-biderman23a} in efficiency and problem-solving capabilities.
% 2024， OLMo (Open Language Model) \cite{groeneveld2024olmo}  发布 OLMo 以及开放训练数据以及训练和评估代码 \footnote{https://allenai.org/olmo}。发布的模型包括 7B 规模的语言模型的四种变体，对应于不同的架构、优化器和训练硬件，以及一种 1B 规模(16 layers, 2048 dimension, 2T tokens)的模型，全部都在至少 2T 令牌上进行训练。采用基于解码器的transformer架构. 遵循 LLaMA、PaLM 等，我们从架构中排除所有偏差项，以提高训练稳定性。使用层范数的非参数公式。使用 SwiGLU 激活函数。用旋转位置嵌入替换绝对位置嵌入。最终词汇量为50,280。构建并发布了我们的预训练数据集 Dolma。表 \ref{tab:olmo_model_performance} 总结了 OLMo 的零样本评估结果，并与其他同等规模的公开可用模型进行了比较。报告评估套件中 8 项核心任务(arc (both arc_easy and arc_challenge) \cite{clark2018think}, boolq \cite{clark2019boolq}, openbookqa \cite{mihaylov2018can}, sciq \cite{welbl2017crowdsourcing}, hellaswag \cite{zellers2019hellaswag}, piqa \cite{bisk2020piqa}, and winogrande \cite{sakaguchi2021winogrande})的结果。
The \textbf{Open Language Model (OLMo)} \cite{groeneveld2024olmo} has been released with its training data, code, and evaluation metrics available at \footnote{https://allenai.org/olmo}. It includes four 7B-scale language models with various architectures, optimizers, and hardware setups, alongside a 1B model (16 layers, 2048 dimension, trained on 2T tokens). These models, leveraging a decoder-based transformer architecture, exclude bias terms to enhance stability and use non-parametric layer normalization and SwiGLU activations. Rotary positional embeddings replace absolute ones, and the vocabulary is set at 50,280. The Dolma dataset supports their training. Table \ref{tab:olmo_model_performance} presents OLMo’s zero-shot performance on eight tasks: ARC \cite{clark2018think}, BoolQ \cite{clark2019boolq}, OpenBookQA \cite{mihaylov2018can}, SciQ \cite{welbl2017crowdsourcing}, HellaSwag \cite{zellers2019hellaswag}, PIQA \cite{bisk2020piqa}, and Winogrande \cite{sakaguchi2021winogrande}, comparing it against other models of similar size.
\begin{table}[ht]
\centering
\caption{Zero-shot evaluation of OLMo-1B and OLMo-7B, with other publicly available comparable model checkpoints on 8 core tasks from the downstream evaluation suite described in Section 2.4. For OLMo-7B, we report results for the 2.46T token checkpoint.}
\label{tab:olmo_model_performance}
\begin{tabular}{lcccccccccc}
\hline
\textbf{Models} & \textbf{arc challenge} & \textbf{arc easy} & \textbf{boolq} & \textbf{hella-swag} & \textbf{open bookqa} & \textbf{piqa} & \textbf{sciq} & \textbf{wino-grande} & \textbf{avg.} \\
\hline
StableLM 1.6B   & 43.8 & 63.7 & 76.6 & 68.2 & 45.8 & 74.0 & 94.7 & 64.9 & 66.5 \\
Pythia 1B       & 33.1 & 50.2 & 61.8 & 44.7 & 37.8 & 69.1 & 86.0 & 53.3 & 54.5 \\
TinyLlama 1.1B  & 34.8 & 53.2 & 64.6 & 58.7 & 43.6 & 71.1 & 90.5 & 58.9 & 59.4 \\
OLMo-1B         & \textbf{34.5} & \textbf{58.1} & \textbf{60.7} & \textbf{62.5} & \textbf{46.4} & \textbf{73.7} & \textbf{88.1} & \textbf{58.9} & \textbf{60.4} \\
Falcon-7B       & 47.5 & 70.4 & 74.6 & 75.9 & 53.0 & 78.5 & 93.9 & 68.9 & 70.3 \\
LLaMA 7B        & 44.5 & 67.9 & 75.4 & 76.2 & 51.2 & 77.2 & 93.9 & 70.5 & 69.6 \\
Llama 2 7B      & 48.5 & 69.5 & 80.2 & 76.8 & 48.4 & 76.7 & 94.5 & 69.4 & 70.5 \\
MPT-7B          & 46.5 & 70.5 & 74.2 & 77.6 & 48.6 & 77.3 & 93.7 & 69.9 & 69.8 \\
Pythia 6.9B     & 44.1 & 61.9 & 61.1 & 63.8 & 45.0 & 75.1 & 91.1 & 62.0 & 63.0 \\
RPJ-INCITE-7B   & 42.8 & 68.4 & 68.6 & 70.3 & 49.4 & 76.0 & 92.9 & 64.7 & 66.6 \\
OLMo-7B         & \textbf{48.5} & \textbf{65.4} & \textbf{73.4} & \textbf{76.4} & \textbf{50.4} & \textbf{78.4} & \textbf{93.8} & \textbf{67.9} & \textbf{69.3} \\
\hline
\end{tabular}
\end{table}
% 2023 Cerebras-GPT \cite{dey2023cerebras}, 参数范围从 111M 扩展到 13B, 在 Eleuther Pile 数据集上训练 Cerebras-GPT 模型，以实现高效的预训练. Pre-trained models are available on HuggingFace: \footnote{https://huggingface.co/cerebras}. The source code is available in the Cerebras Modelzoo: \footnote{https://github.com/Cerebras/modelzoo}. 测试并发现，每个参数使用大约 20 个标记进行训练的模型提供了计算效率最高的预训练，与 Chinchilla 结果一致。使用 FP16 混合精度和 bfloat16 精度训练模型。随着标准训练模型规模的扩大，它们往往会变得不稳定，因为权重和激活值会达到用于训练它们的数值表示的限制。为了解决这些问题，还训练了一组具有最大更新参数化 (μP) 的 CerebrasGPT 模型。除了提高训练稳定性之外，μP 还提高了训练超参数从小规模模型到大规模模型的可迁移性，这种技术称为 μTransfer。使用 EleutherAI 评估工具，在零样本和五样本设置下的一套七个常识推理任务(HellaSwag, PIQA, WinoGrande, Lambada, ARC (both the easy and challenge versions), and OpenBookQA)上评估 Cerebras-GPT 和公开可用的模型\cite{gao10256836framework}。comparing Cerebras-GPT to GPT-J, GPT-NeoX, and Pythia, 在相同的FLOPs下， Cerebras-GPT总是能够实现更低的pre-training loss，具有更高的效率。
\textbf{Cerebras-GPT} \cite{dey2023cerebras}, with parameters ranging from 111M to 13B, was trained on the EleutherAI Pile dataset for efficient pre-training. Pre-trained models are available on HuggingFace \footnote{https://huggingface.co/cerebras}. Source code is accessible at the Cerebras Modelzoo \footnote{https://github.com/Cerebras/modelzoo}. It was found that training each parameter with approximately 20 tokens provided the highest computational efficiency, consistent with the Chinchilla study. Models were trained using FP16 mixed precision and bfloat16 precision. As model sizes increased, they tended to become unstable due to the numerical limits of weights and activations. To mitigate these issues, a set of Cerebras-GPT models with Maximum Update Parametrization (\(\mu\)P) was also trained. This technique, \(\mu\)Transfer, not only enhances training stability but also improves the transferability of training hyperparameters across different model scales. Cerebras-GPT was evaluated using EleutherAI's tools on a suite of seven common-sense reasoning tasks (HellaSwag, PIQA, WinoGrande, Lambada, ARC (both easy and challenging versions), and OpenBookQA) in zero-shot and few-shot settings, comparing its performance with GPT-J, GPT-NeoX, and Pythia. Across comparable FLOPs, Cerebras-GPT consistently achieved lower pre-training losses and demonstrated higher efficiency.
% 2023 Pythia \cite{pmlr-v202-biderman23a} 一套仅限解码器的自回归语言模型，参数范围从 70M 到 12B，专门为促进此类科学研究而设计。 Trained models, analysis code, training code, and training data can be found at https: //github.com/EleutherAI/pythia. 在 Pile \cite{gao2020pile}上和重复数据删除后的 Pile 上分别训练 8 个模型大小，train all models for 300B tokens, 提供 2 个可以比较的套件副本。对我们的模型使用完全密集的层。训练期间的 Flash Attention \cite{dao2022flashattention}可提高设备吞吐量。使用\citet{su2024roformer}引入的旋转嵌入并且现在被广泛使用作为我们选择的位置嵌入类型。使用 \citet{wang2022gpt}引入的并行注意力和前馈技术以及模型初始化方法. 使用 Adam 进行训练，并利用零冗余优化器 (ZeRO)\cite{rajbhandari2020zero}来有效地扩展到多机设置。我们还适当利用数据并行性\cite{goyal2017accurate}和张量并行性\cite{shoeybi2019megatron}来优化性能。Pythia 和 Pythia（重复数据删除）在各种 NLP 基准测试(The task names listed in the image are: Lambada (OpenAI), PIQA, WinoGrande, WSC, ARC - Easy, ARC - Challenge, SciQ, LogiQA)中的表现与 OPT 和 BLOOM 模型非常相似。
\textbf{Pythia} \cite{pmlr-v202-biderman23a}, an autoregressive language model exclusively designed for scientific research, features model sizes ranging from 70M to 12B parameters. Comprehensive resources including training models, analysis code, training code, and datasets are available at https://github.com/EleutherAI/pythia. It was trained on the Pile \cite{gao2020pile} and its deduplicated version, across eight model sizes for 300 billion tokens. Models utilize fully dense layers and Flash Attention \cite{dao2022flashattention} to enhance throughput. They incorporate rotational embeddings introduced by \citet{su2024roformer} and use parallel attention, feed-forward techniques, and model initialization methods from \citet{wang2022gpt}. Training employs the Adam optimizer and leverages the Zero Redundancy Optimizer (ZeRO) \cite{rajbhandari2020zero} for effective multi-machine scaling. Data \cite{goyal2017accurate} and tensor \cite{shoeybi2019megatron} parallelism are optimized for performance. Pythia's performance on NLP benchmarks including Lambada (OpenAI), PIQA, WinoGrande, WSC, ARC - Easy, ARC - Challenge, SciQ, and LogiQA parallels that of OPT and BLOOM models.
% 2022 OPT \cite{zhang2022opt} 仅限解码器的预训练 Transformer，参数范围从 125M (12 layers, 768 dimension), 350M, 1.3B, 2.7B, 5.7B,...最大到 175B. 预训练语料库包含 RoBERTa \cite{liu2019roberta}、Pile \cite{gao2020pile} 和 PushShift.io Reddit \cite{baumgartner2020pushshift} 中使用的数据集串联, 主要是英文文本，我们的最终语料库包含大约 180B 个标记。根据文献中使用的 16 个标准 NLP 任务评估我们的模型：HellaSwag \ref{zellers2019hellaswag}、StoryCloze \cite{mostafazadeh2016corpus}、PIQA \cite{bisk2020piqa}、ARC Easy 和 Challenge \cite{clark2018think}、OpenBookQA \cite{mihaylov2018can}、WinoGrad \cite{levesque2012winograd}、WinoGrande \cite{sakaguchi2021winogrande}和 SuperGLUE \cite{wang2019superglue}。实验结果(Fig. \ref{fig:opt_exp})显示，opt和gpt在不同的model size上表现相当， zero-shot和few-shot场景下。code is here \footnote{https://github.com/facebookresearch/metaseq/tree/main/projects/OPT}. 
\textbf{OPT} \cite{zhang2022opt}, a decoder-only pre-trained Transformer, spans model sizes from 125M (12 layers, 768 dimensions) to 175B. It's trained on a corpus combining data from RoBERTa \cite{liu2019roberta}, Pile \cite{gao2020pile}, and PushShift.io Reddit \cite{baumgartner2020pushshift}, mostly in English, totaling around 180 billion tokens. OPT is assessed using 16 standard NLP tasks such as HellaSwag \cite{zellers2019hellaswag}, StoryCloze \cite{mostafazadeh2016corpus}, PIQA \cite{bisk2020piqa}, ARC \cite{clark2018think}, OpenBookQA \cite{mihaylov2018can}, WinoGrad \cite{levesque2012winograd}, WinoGrande \cite{sakaguchi2021winogrande}, and SuperGLUE \cite{wang2019superglue}. Results (Fig. \ref{fig:opt_exp}) show OPT matches GPT across sizes in zero-shot and few-shot scenarios. Code available \footnote{https://github.com/facebookresearch/metaseq/tree/main/projects/OPT}.
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.5\linewidth]{Pic/model/opt_exp.png}
    \caption{Multi-shot performance. OPT performance for one- and few-shot lags behind GPT-3 models, but performance depends heavily per task}
    \label{fig:opt_exp}
\end{figure}
% 2022. XGLM~\cite{lin-etal-2022-shot}, 考虑语言模型的\textbf{多语言小样本学习能力}。使用包含 30 种不同语言的 500B 个令牌的大规模语料库来训练模型，对资源较少的语言进行上采样以呈现更平衡的语言表示。评估多个多语言自然语言理解 (NLU) 任务、机器翻译和英语任务子集的模型 in \cite{NEURIPS2020_1457c0d6}。four models with 564M (24 layers, 1024-dimension, 相同的结构比GPT更大是因为更大的词表带来更大的embedding参数量), 1.7B, 2.9B, and 7.5B parameters。预训练数据扩展用于挖掘 CC100 语料库\cite{wenzek2020ccnet}的管道以生成 CC100-XL，这是一个更大的多语言数据集，涵盖 68 个 Common Crawl (CC) 快照和 134 种语言。decoder-only causal language models with the Transformer architecture similar to GPT-3. 评估在四个多语言任务，涵盖常识推理 (XCOPA)、照应解析 (XWinograd)、自然语言推理 (XNLI) 和释义 (PAWSX)。\ref{xglm_scaling_up}显式模型越大，越好的利用in-context example，也显式564M已经显式出了emergent ability在这些下游任务上。code is here \footnote{https://github.com/facebookresearch/ fairseq/tree/main/examples/xglm}.
\textbf{XGLM}~\cite{lin-etal-2022-shot} focuses on multilingual few-shot learning, trained with a massive corpus of 500 billion tokens across 30 languages. The training involved up-sampling under-resourced languages to ensure balanced linguistic representation. This model has been evaluated on multiple multilingual natural language understanding tasks, machine translation, and subsets of English tasks \cite{NEURIPS2020_1457c0d6}. XGLM configurations include four sizes: 564M (24 layers, 1024 dimensions), 1.7B, 2.9B, and 7.5B parameters. The training leveraged an expanded dataset, CC100-XL, derived from CC100 \cite{wenzek2020ccnet}, which includes data from 68 Common Crawl snapshots and covers 134 languages. These decoder-only, Transformer-based causal language models similar to GPT-3 were assessed on tasks including commonsense reasoning (XCOPA), coreference resolution (XWinograd), natural language inference (XNLI), and paraphrase detection (PAWSX). The results \ref{xglm_scaling_up} show that larger models more effectively utilize in-context examples, and the 564M model exhibits emergent abilities on these downstream tasks. Code is available here \footnote{https://github.com/facebookresearch/fairseq/tree/main/examples/xglm}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\linewidth]{Pic/model/xglm_scaling_up.png}
    \caption{Zero-shot and in-language few-shot learning performance as a function of model size. The last plot shows the average performance over all five tasks in 0and 4-shot learning.}
    \label{fig:xglm_scaling_up}
\end{figure}
% 2021 GPT-Neo \cite{gpt-neo} \footnote{https://github.com/EleutherAI/gpt-neo}, An implementation of model parallel GPT-2 and GPT-3-style models using the mesh-tensorflow library. size includes 125M (12 layers, 768-dimension), 350M (24 layers, 1024-dimension), 1.3B, 2.7B. 窗口大小256，词表大小50257. 使用 Pile 数据集进行训练。GPT Neo 的小规模和其自然语言理解和生成能力使其适合于聊天机器人、虚拟助手和客户支持系统等任务。
\textbf{GPT-Neo} \cite{gpt-neo} \footnote{\url{https://github.com/EleutherAI/gpt-neo}}, introduced in 2021, utilizes mesh-tensorflow for model-parallel GPT-2 and GPT-3 architectures. Variants range from 125M to 2.7B parameters, trained on the Pile dataset, excelling in tasks for chatbots, virtual assistants, and customer support due to its robust natural language capabilities.
% 2019 \cite{shoeybi2019megatron} megatron-gpt2. code is here \footnote{https://github.com/ NVIDIA/Megatron-LM}. 创建一个由 Wikipedia \cite{devlin2019bert}、CC-Stories \cite{trinh2018simple}、RealNews \cite{zellers2019defending} 和 OpenWebtext \footnote{https://openai.com/blog/ better-language-models/} 组成的聚合数据集。对于 BERT 模型，我们在训练数据集中包含 BooksCorpus \cite{zhu2015aligning}，但是，该数据集被排除在 GPT-2 训练之外，因为它与 LAMBADA 任务重叠 (SOTA来自于数据集的重新编译)。生成的聚合语料库包含 174 GB 的重复数据删除文本。所有的实验均使用多达 32 台 DGX-2H 服务器（总共 512 个 Tesla V100 SXM3 32GB GPU）。vocabulary size of 51,200. 文章考虑了GPT类型和BERT类型的语言模型。For GPT-2类，有355M （24 layers, 1024 dimension），2.5B (54 layers, 1920 dimension)和8.3B(72 layers, 3072 dimension)几个版本。BERT类包括336M，1.3B，和3.9B几个版本。对几个下游任务的训练模型进行了微调，包括来自 GLUE 基准的 MNLI 和 QQP \cite{wang2018glue}、来自斯坦福问答数据集的 SQuAD 1.1 和 SQuAD 2.0 \cite{rajpurkar2016squad}以及阅读理解 RACE 数据集 \cite{lai2017race}。实验结果显示随着模型大小的增加，下游任务性能在所有情况下都会得到改善，(b) 与其他基于 BERT 的模型相比，我们的 3.9B 模型在开发集上建立了最先进的结果。
\citet{shoeybi2019megatron} developed \textbf{Megatron-GPT2}, with code available at \footnote{\url{https://github.com/NVIDIA/Megatron-LM}}. They assembled a dataset from Wikipedia \cite{devlin2019bert}, CC-Stories \cite{trinh2018simple}, RealNews \cite{zellers2019defending}, and OpenWebtext \footnote{\url{https://openai.com/blog/better-language-models/}}. For BERT models, the training set included BooksCorpus \cite{zhu2015aligning}, but it was excluded from GPT-2 training to prevent overlap with the LAMBADA task. The combined corpus contains 174 GB of deduplicated text. Experiments utilized up to 32 DGX-2H servers, totaling 512 Tesla V100 SXM3 32GB GPUs. The GPT-2 versions include 355M (24 layers, 1024 dimensions), 2.5B (54 layers, 1920 dimensions), and 8.3B (72 layers, 3072 dimensions); BERT versions comprise 336M, 1.3B, and 3.9B. Models were fine-tuned on downstream tasks like MNLI and QQP from the GLUE benchmark \cite{wang2018glue}, SQuAD 1.1 and 2.0 \cite{rajpurkar2016squad}, and the RACE dataset \cite{lai2017race}. Results indicate that performance on downstream tasks improves with model size, with the 3.9B model establishing state-of-the-art results on development sets.

% 压缩出来的
% 2024, LaMini-LM \cite{wu2024lamini}, 从大模型中蒸馏出来的模型，采用LLM的序列蒸馏（也称为离线蒸馏）。从不同的现有数据集中整理这些指令，包括 self-instruct \cite{wang2023selfb}、P3 \cite{sanhmultitask}、FLAN \cite{longpre2023flan}和 Alpaca \cite{alpaca}）。为了扩充数据集，使用示例引导指令生成技术和 gpt-3.5-turbo 来生成在风格和质量上与人类书面提示相匹配的其他多样化指令,consisting of over 2.58M examples。还采用主题引导指令生成技术，通过合并维基百科中感兴趣的特定主题来增强指令多样性。利用 gpt-3.5-turbo 为每条指令生成响应。生成的数据集称为 LaMini 指令数据集。微调多个具有不同大小（范围从 61M 到 7B）和架构（编码器解码器和仅解码器）的较小语言模型(T5 \cite{raffel2020exploring}, Flan-T5  \cite{longpre2023flan}, Cerebras-GPT \cite{dey2023cerebras}, GPT-2 \cite{radford2019language}, GPT-Neo \cite{gao2020pile}, GPT-J \cite{gpt-j}, and LLaMA\cite{touvron2023llama2}.)。对下游 NLP 任务的零样本评估, 15 种不同的 NLP 任务，涵盖 QA、情感分析、释义识别、自然语言推理、共指消解、词义消歧和句子补全。这些 NLP 任务的详细信息位于表\ref{tab:downstream_nlp_tasks}。 LaMini-LLaMA-7B 的平均性能，其性能显着优于 LLaMA-7B 和 Alpaca-7B。这些发现凸显了指令数据集的重要意义。
\textbf{LaMini-LM }\cite{wu2024lamini} distills from large models through sequence distillation, utilizing diverse instructions from datasets like self-instruct \cite{wang2023selfb}, P3 \cite{sanhmultitask}, FLAN \cite{longpre2023flan}, and Alpaca \cite{alpaca}. Enhanced with example-guided techniques and gpt-3.5-turbo, the LaMini Instruction Dataset includes over 2.58M examples crafted to match human-written prompts. This dataset aided in fine-tuning smaller language models, ranging from 61M to 7B parameters, across various architectures including T5 \cite{raffel2020exploring}, Flan-T5 \cite{longpre2023flan}, Cerebras-GPT \cite{dey2023cerebras}, GPT-2 \cite{radford2019language}, GPT-Neo \cite{gao2020pile}, GPT-J \cite{gpt-j}, and LLaMA \cite{touvron2023llama2}. Zero-shot performance on 15 diverse NLP tasks—covering QA, sentiment analysis, paraphrase identification, natural language inference, co-reference resolution, word sense disambiguation, and sentence completion—is documented in Table \ref{tab:downstream_nlp_tasks}. LaMini-LLaMA-7B notably surpassed LLaMA-7B and Alpaca-7B, underscoring the instructional dataset’s impact.

\begin{table}[!h]
\centering
\begin{tabular}{lllcc}
\hline
\textbf{Task Category} & \textbf{Dataset} & \textbf{Size} & \textbf{Metric} \\
\hline
Multiple-Choice QA & OpenBookQA \cite{mihaylov2018can} & 500 & Accnorm \\
 & SciQ \cite{welbl2017crowdsourcing} & 1,000 & Accnorm \\
 & RACE \cite{lai2017race} & 1,045 & Acc \\
 & ARC \cite{clark2018think} & 1,172 & Accnorm \\
 & PIQA \cite{bisk2020piqa} & 1,838 & Accnorm \\
\hline
Extractive QA & ReCoRD \cite{zhang2018record} & 10,000 & F1 \\
\hline
Sentiment Analysis & SST \cite{socher2013recursive} & 872 & Acc \\
\hline
Paraphrase Identification & MRPC \cite{dolan2005automatically} & 408 & Acc \\
\hline
Natural Language Inference & RTE \cite{wang2018glue} & 277 & Acc \\
 & MultiNLI \cite{williams-etal-2018-broad} & 9,815 & Acc \\
 & MultiNLI (mis) \cite{williams-etal-2018-broad} & 9,832 & Acc \\
\hline
Coreference Resolution & WSC273 \cite{levesque2012winograd} & 273 & Acc \\
 & WinoGrande \cite{sakaguchi2021winogrande} & 1,267 & Acc \\
\hline
Word Sense disambiguation & WiC \cite{pilehvar2019wic} & 638 & Acc \\
\hline
Sentence Completion & HellaSwag \cite{zellers2019hellaswag} & 10,042 & Accnorm \\
\hline
\end{tabular}
\caption{Details of 15 downstream NLP tasks. Accnorm indicates the target sequence length and normalizes the output probability used for computing the accuracy.}
\label{tab:downstream_nlp_tasks}
\end{table}
% 【质量低下】2023 Orca \cite{mitra2023orca} 提出了一个教小模型的策略：prompt erasing，在行为克隆上面进行了改进，设计了任务特定的系统提示，但是微调小模型时候不让它看见。orca 2有7b和13b两个版本，基于llama7b和13b的。code is here \footnote{aka.ms/orca-lm}. 创建了一个包含约 817K 训练实例的新数据集，我们将其称为 Orca 2 数据集, 包括FLAN-v2 \cite{longpre2023flan}, Orac 1, 和GPT-4生成的数据。从 LLaMA-2-7B 或 LLaMA-2-13B 检查点开始，并在一个 epoch 的 FLAN-v2 数据集的训练分割上对其进行微调。请注意，FLAN-v2 数据集包含零样本和少样本问题。然后，我们使用来自 Orca 1 的 500 万个 ChatGPT 数据进行 3 个 epoch 的训练。然后，我们使用 Orca 1 的 100 万个 GPT-4 数据和 Orca 2 的 817K 数据组合进行 4 个 epoch 的训练。使用 bfloat16 在 32 个 80GB 内存的 NVIDIA A100 GPU 上训练 Orca 2。详细概述了为评估 Orca 2 的开放式生成、总结、安全性、偏见、推理和理解能力而选择的任务。Orca-2-7B 在所有推理任务上都优于或与 LLaMA-2-Chat-70B 相当。
\textbf{Orca} \cite{mitra2023orca} introduces a teaching strategy for small models known as "prompt erasing," improving upon behavior cloning by designing but hiding task-specific prompts during model fine-tuning. Orca 2 is available in two sizes, 7B and 13B, based on LLaMA-7B and LLaMA-13B respectively. The source code can be found here \footnote{aka.ms/orca-lm}. A new dataset, the Orca 2 dataset, was developed, comprising about 817K training instances from FLAN-v2 \cite{longpre2023flan}, Orca 1, and data generated by GPT-4. The models are fine-tuned starting from LLaMA-2-7B or LLaMA-2-13B checkpoints on FLAN-v2 dataset’s training split for one epoch, covering zero-shot and few-shot problems, followed by three epochs on 5 million ChatGPT data from Orca 1 and four epochs combining 1 million GPT-4 data with 817K Orca 2 data. Training occurred using bfloat16 across 32 NVIDIA A100 GPUs with 80GB each. The evaluation tasks for assessing Orca 2’s capabilities in open-ended generation, summarization, safety, bias, reasoning, and comprehension are extensively detailed. Orca-2-7B matches or exceeds LLaMA-2-Chat-70B across all assessed reasoning tasks.

% 另一个版本的介绍，在QA task from scratch
Orac 1~\cite{mukherjee2023orca} enhances LLM responses through explanation tuning, utilizing a mix of tasks from FLAN-v2~\cite{longpre2023flan}. Each task includes a system prompt, user prompt, and LLM response. To vary response diversity, 16 crafted system prompts are designed to guide LLM behavior. For data construction, Orac 1 employs ChatGPT to generate 5M instructions (named FLAN-5M) and GPT-4~\cite{achiam2023gpt} for an additional 1M queries (named FLAN-1M). Orac 1 trained for 160 hours on FLAN-5M and 40 hours on FLAN-1M. Its evaluation (we extract only a small portion of the experiments from the original paper, similar to the following paragraphs.) across a range of professional and academic exams in QA format, including GRE, GMAT, LSAT, and SAT from the AGIEval benchmark~\cite{zhong2024agieval} in zero-shot settings shows Orac 1 narrows the performance gap with foundation models to only 5 points against ChatGPT.

% [好文章]
% FlanT5 + Specialized \cite{fu2023specializing} 提出一种专业化小模型的方法来激发在特定任务上的emergent ability. 如果模型规模较小（根据经验小于 100B 参数），CoT 会表现出平坦，有时甚至接近于零的缩放曲线. 在达到某个阈值之前，模型 CoT 性能从扩展中获益甚少，如图\ref{fig:specializing_scaling_curving}(a)所示。一个经典的emergent ability是perform multi-step reasoning on math work problems with cot prompting，因此本文以数学推理任务为例。小模型（≤10B）的模型容量有限，但如果将其容量“集中”在一个目标任务上（以降低其他任务的能力为代价改进一项目标任务），模型可以获得不错的性能提升。通过从大型教师模型（GPT-3.5 codedavinci-002 \cite{chen2021evaluating}）中提取 GSM8K 数据的思想链推理路径来微调指令调整模型（FlanT5 \cite{chung2024scaling}）。大幅改善小型 FlanT5 模型（250M、760M 和 3B）上 CoT 推理的扩展趋势（平均 +10 准确度增益）在一组 4 项数学推理任务（1 个分布内和 3 个分布外）上, 如表\ref{tab:specialize_flant5_performance}所示。直接在 CoT 数据上进行训练还可以将原始 T5 检查点的平坦缩放曲线（图\ref{fig:specializing_scaling_curving}(B)）提升为对数线性。specialization显着提升了  FlanT5 的缩放曲线，并且两条曲线也是对数线性的 （图\ref{fig:specializing_scaling_curving}(c)）。code is here \footnote{https://github.com/ FranxYao/FlanT5-CoT-Specialization}
FlanT5 + Specialized \cite{fu2023specializing} introduces a method to specialize small models, fostering emergent abilities in specific tasks. It finds that models smaller than 100B parameters exhibit flat scaling curves for CoT until a certain threshold, beyond which performance gains are minimal, as illustrated in Figure \ref{fig:specializing_scaling_curving}(a). The study focuses on mathematical reasoning tasks, demonstrating that concentrating a model's capacity on a single target task can significantly enhance performance. The method involves fine-tuning the FlanT5 \cite{chung2024scaling} model using chains of thought from a larger GPT-3.5 codedavinci-002 \cite{chen2021evaluating} model, which improves CoT reasoning on the FlanT5 models (250M, 760M, 3B), achieving an average +10 accuracy gain across four math tasks, as shown in Table \ref{tab:specialize_flant5_performance}. Training directly on CoT data also transforms the original flat scaling curve of the T5 checkpoint into a logarithmic linear trend, significantly boosting FlanT5’s scaling curves, as depicted in Figure \ref{fig:specializing_scaling_curving}(b and c). Access the code for this study here \footnote{https://github.com/FranxYao/FlanT5-CoT-Specialization}.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{Pic/model/specializing_scaling_curving.png}
    \caption{X-axis means log of model scale, y-axis means validation accuracy on GSM8K. A: Previously, the community believed that small models have flat curves for both AO and CoT prompting and only when models become large enough the performance will have a “phase change” and suddenly increase. B: we show that after training on CoT, the model exhibits log-linear curves where both AO and CoT increase with the model scale. C: for instruction-tuned models (FlanT5) that already exhibit CoT, specialization lifts up the scaling curve, and the two curves are again, log-linear shaped. All the log-linear curves indicate that chain-of-thought may not be an emergent ability which is marked by the flat-then-phase-change curve. Here we show the curve on a small scale is not flat but actually log-linear, and continuously increasing model scale leads to continuously increased accuracy (no sudden phase change).}
    \label{fig:specializing_scaling_curving}
\end{figure}
\begin{table}[h]
\centering
\caption{Overall test set performance. We specialize Flan-T5's ability from generic tasks (BigBench Hard) to math reasoning tasks.}
\label{tab:specialize_flant5_performance}
\begin{tabular}{lcccccccccc}
\hline
\textbf{Models} & \textbf{\#Params} & \textbf{GSM8K} & \textbf{MultiArith} & \textbf{ASDiv} & \textbf{SVAMP} & \textbf{AO} & \textbf{CoT} & \textbf{Acc.} & \textbf{$\Delta$} \\
\hline
code-DaVinci-002 & >175B & 63.1 & 95.8 & 80.4 & 76.4 & 56.6 & 73.9 & - & - \\
LaMDA & 137B & 14.8 & 45.0 & 46.6 & 37.5 & 37.4 & 43.0 & - & - \\
PaLM & 60B & 29.9 & 75.0 & 61.9 & 46.7 & - & - & - & - \\
UL2 & 20B & 4.4 & - & 16.9 & 12.5 & - & - & - & - \\
\textbf{FlanT5-XXL + Specialized} & 11B & 27.1 & 63.0 & 37.6 & 35.6 & 19.6 & 0.0 & +11.0 & -41.8 \\
\textbf{FlanT5-XL + Specialized} & 3B & 22.4 & 42.3 & 28.4 & 23.8 & 3.2 & 0.0 & +8.9 & -35.8 \\
\textbf{FlanT5-Large + Specialized} & 760M & 20.2 & 38.5 & 23.8 & 20.4 & 6.5 & 0.3 & +13.3 & -30.6 \\
\textbf{FlanT5-Base + Specialized} & 250M & 13.4 & 29.7 & 20.9 & 14.2 & 3.1 & 0.1 & +10.4 & -25.8 \\
\hline
\end{tabular}
\end{table}
% 2022 FlanT5 \cite{chung2024scaling}. 在以指令形式表达的数据集集合上微调语言模型可以提高模型性能和对未见过的任务的泛化。Code is here \footnote{https://github.com/google-research/t5x/blob/main/docs/models.md# flan-t5-checkpoints.}. 通过结合先前工作中的四种混合物，可扩展至 1,836 个微调任务：Muffin、T0-SF、SNI 和 CoT，如图\ref{flan_dataset} 所示。用以下具有挑战性的基准。 (1) MMLU \cite{hendrycksmeasuring包括数学、历史、法律和医学等 57 项任务的考试题。 (2) BBH 包括来自 BIG-Bench 的 23 项具有挑战性的任务\cite{srivastava2023beyond}。 (3) TyDiQA \cite{clark2020tydi}是跨 8 种类型不同语言的问答基准。 (4) MGSM \cite{shilanguage}是提出的数学应用题的多语言基准,手动翻译成 10 种语言。表\ref{tab:flan_exp}显示，指令调优之后的模型效果更好。
\textbf{FlanT5} \cite{chung2024scaling} improves performance and generalization to new tasks by fine-tuning language models on instruction-based datasets. Access the code here \footnote{https://github.com/google-research/t5x/blob/main/docs/models.md\#flan-t5-checkpoints}. It incorporates four task mixtures—Muffin, T0-SF, SNI, and CoT—spanning 1,836 fine-tuning tasks, as depicted in Figure \ref{flan_dataset}. The model is evaluated using challenging benchmarks: (1) MMLU \cite{hendrycksmeasuring}, covering 57 tasks across domains such as mathematics, history, law, and medicine; (2) BBH from BIG-Bench \cite{srivastava2023beyond} with 23 tasks; (3) TyDiQA \cite{clark2020tydi}, a QA benchmark in eight diverse languages; and (4) MGSM \cite{shilanguage}, a multilingual benchmark for math problems, translated into 10 languages. Results in Table \ref{tab:flan_exp} indicate superior performance of instructionally tuned models.
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{Pic/model/flan_dataset.png}
    \caption{finetuning data comprises 473 datasets, 146 task categories, and 1,836 total tasks.}
    \label{fig:flan_dataset}
\end{figure}
\begin{table}[htbp]
\centering
\begin{tabular}{|c|l|c|c|c|c|c|c|}
\hline
\textbf{Params} & \textbf{Model} & \textbf{Norm. avg.} & \multicolumn{2}{c|}{\textbf{MMLU}} & \multicolumn{2}{c|}{\textbf{BBH}} & \textbf{MGSM} \\
\hline
& & & \textbf{Direct} & \textbf{CoT} & \textbf{Direct} & \textbf{CoT} & \textbf{CoT} \\
\hline
80M  & T5-Small       & -9.2 & 26.7 & 5.6  & 27.0 & 7.2  & 0.4 \\
     & Flan-T5-Small  & -3.1 (+6.1) & 28.7 & 12.1 & 29.1 & 19.2 & 0.2 \\
\hline
250M & T5-Base        & -5.1 & 25.7 & 14.5 & 27.8 & 14.6 & 0.5 \\
     & Flan-T5-Base   & 6.5 (+11.6) & 35.9 & 33.7 & 31.3 & 27.9 & 0.4 \\
\hline
780M & T5-Large       & -5.0 & 25.1 & 15.0 & 27.7 & 16.1 & 0.7 \\
     & Flan-T5-Large  & 13.8 (+18.8) & 45.1 & 40.5 & 37.5 & 31.5 & \\
\hline
3B   & T5-XL          & -4.1 & 25.7 & 14.5 & 27.4 & 19.2 & \\
     & Flan-T5-XL     & 19.1 (+23.2) & 52.4 & 45.5 & 41.0 & 35.2 & \\
\hline
11B  & T5-XXL         & -2.9 & 25.9 & 18.7 & 29.5 & 19.3 & 1.0 \\
     & Flan-T5-XXL    & 23.7 (+26.6) & 55.1 & 48.6 & 45.3 & 41.8 & 4.9 \\
\hline
\end{tabular}
\caption{Instruction finetuning (Flan) improves performance compared to other continued pretraining methods. The benchmark suites are MMLU (57 tasks), BBH (23 tasks), TyDiQA (8 languages), and MGSM (10 languages). The evaluation metric on all four benchmark suites is few-shot prompted accuracy (exact match), where we take an unweighted average overall task. As an aggregate metric, we report the normalized average of MMLU-direct, MMLU-CoT, BBH-direct, BBH-CoT, TyDiQA, and MGSM. These evaluation benchmarks are held out (not included in the finetuning data).}
\label{tab:flan_exp}
\end{table}
